Fragments to Facts: Partial-Information Fragment Inference from LLMs

Large language models (LLMs) can leak sensitive training data through memorization and membership inference attacks. Prior work has primarily focused on strong adversarial assumptions, including attacker access to entire samples or long, ordered prefixes, leaving open the question of how vulnerable LLMs are when adversaries have only partial, unordered sample information. For example, if an attacker knows a patient has "hypertension," under what conditions can they query a model fine-tuned on patient data to learn the patient also has "osteoarthritis?" In this paper, we introduce a more general threat model under this weaker assumption and show that fine-tuned LLMs are susceptible to these fragment-specific extraction attacks. To systematically investigate these attacks, we propose two data-blind methods: (1) a likelihood ratio attack inspired by methods from membership inference, and (2) a novel approach, PRISM, which regularizes the ratio by leveraging an external prior. Using examples from both medical and legal settings, we show that both methods are competitive with a data-aware baseline classifier that assumes access to labeled in-distribution data, underscoring their robustness.

==> sections/limitations.tex <==
\section{Limitations}\label{sec:limitations} 

We acknowledge that the present work offers only a limited treatment of the efficacy of differentially private fine-tuning to protect against attacks under PIFI. We note, however, that though understanding the impact of DP is important for settings where developers are mindful of the possibility of such attacks, fine-tuning LLMs using DP frameworks is far from the norm in practice, in part because of the technical burden of training open LLMs with large batch sizes on a single GPU; 80GB is often needed for fine-tuning with sufficient batch sizes for 8B-parameter models, even after using techniques like qLoRA to reduce memory requirements. This remains a central issue for DP-fine-tuning, which necessitates large capital expenditures that many organizations are not willing to commit. It is a problem that we, as researchers who study these threat models and defenses, have had to contend with in extending our experiments to include models trained under DP. We thus adopt a similar perspective to much prior work in memorization and extraction: though DP fine-tuning may reduce the vulnerability of LLMs to our attacks, this does not diminish the practical importance of the PIFI framework and attacks like PRISM for the majority of fine-tuned LLMs, which do not fine-tune under DP.

